Implicit Conversion of Manifold B-Rep Solids by Neural Halfspace Representation

We present a novel implicit representation -- neural halfspace representation (NH-Rep), to convert manifold B-Rep solids to implicit representations. NH-Rep is a Boolean tree built on a set of implicit functions represented by the neural network, and the composite Boolean function is capable of representing solid geometry while preserving sharp features. We propose an efficient algorithm to extract the Boolean tree from a manifold B-Rep solid and devise a neural network-based optimization approach to compute the implicit functions. We demonstrate the high quality offered by our conversion algorithm on ten thousand manifold B-Rep CAD models that contain various curved patches including NURBS, and the superiority of our learning approach over other representative implicit conversion algorithms in terms of surface reconstruction, sharp feature preservation, signed distance field approximation, and robustness to various surface geometry, as well as a set of applications supported by NH-Rep.

==> figures/patchmerging.tex <==
\begin{figure}[t]
    \centering
    \vspace{3pt}
    \begin{overpic}[width=0.95\columnwidth]{patchmerge_0515}
        \put(0,-6.5){\small before merging}
        \put(29,-6.5){\small after merging}
        \put(55,-6.5){\small after merging}
        \put(3,-3.5){\small Point cloud}
        \put(30,-3.5){\small Point cloud}
        \put(60,-3.5){\small Ours}
        \put(80,-3.5){\small Ground truth}

        \put(0,44){\small {\textbf{\#patches: 168}}}
        \put(28,44){\small {\textbf{\#patches: 13}}}

        \put(0,25){\small {\textbf{\#patches: 158}}}
        \put(28,25){\small {\textbf{\#patches: 8}}}

    \end{overpic}\vspace{5pt}
    \caption{Patch merging for NH-Rep. From left to right: sampled point cloud before and after patch merging, the zero surface of NH-Rep after patch merging and ground truth. NH-Rep can fit the shape accurately after patch merging. }
    \label{fig:patchmerging}
\end{figure}
